Follow the Rules: Reasoning for Video Anomaly Detection with Large Language Models

Video Anomaly Detection (VAD) is crucial for applications such as security surveillance and autonomous driving. However, existing VAD methods provide little rationale behind detection, hindering public trust in real-world deployments. In this paper, we approach VAD with a reasoning framework. Although Large Language Models (LLMs) have shown revolutionary reasoning ability, we find that their direct use falls short of VAD. Specifically, the implicit knowledge pre-trained in LLMs focuses on general context and thus may not apply to every specific real-world VAD scenario, leading to inflexibility and inaccuracy. To address this, we propose AnomalyRuler, a novel rule-based reasoning framework for VAD with LLMs. AnomalyRuler comprises two main stages: induction and deduction. In the induction stage, the LLM is fed with few-shot normal reference samples and then summarizes these normal patterns to induce a set of rules for detecting anomalies. The deduction stage follows the induced rules to spot anomalous frames in test videos. Additionally, we design rule aggregation, perception smoothing, and robust reasoning strategies to further enhance AnomalyRuler's robustness. AnomalyRuler is the first reasoning approach for the one-class VAD task, which requires only few-normal-shot prompting without the need for full-shot training, thereby enabling fast adaption to various VAD scenarios. Comprehensive experiments across four VAD benchmarks demonstrate AnomalyRuler's state-of-the-art detection performance and reasoning ability. AnomalyRuler is open-source and available at: https://github.com/Yuchen413/AnomalyRuler

==> 3_overview.tex <==
\section{Overview}

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figure/VAD.pdf} 
  % \vspace{-0.3in}
  \caption{The \sys pipeline consists of two main stages: induction and deduction. The induction stage involves three modules: i) visual perception processes $n$ sets of normal frames to generate $n$ sets of descriptions; ii) rule generation creates $n$ sets of normal and anomaly rules based on these descriptions; iii) rule refinement employs a voting mechanism for a set of robust rule. The deduction stage also involves three modules: i) the visual perception module analyzes continuous video frames for descriptions; ii) the exponential majority smoothing module adjusts these descriptions considering temporal consistency to ensure neighboring frames share similar characteristics; iii) the reasoning module outputs anomaly detection predictions with reasoning using modified descriptions and robust rules from the induction stage.}\label{fig: pipe}
  % \vspace{-0.3in}
\end{figure}

